Teaching Mining Software Repositories

Mining Software Repositories (MSR) has become a popular research area recently. MSR analyzes different sources of data, such as version control systems, code repositories, defect tracking systems, archived communication, deployment logs, and so on, to uncover interesting and actionable insights from the data for improved software development, maintenance, and evolution. This chapter provides an overview of MSR and how to conduct an MSR study, including setting up a study, formulating research goals and questions, identifying repositories, extracting and cleaning the data, performing data analysis and synthesis, and discussing MSR study limitations. Furthermore, the chapter discusses MSR as part of a mixed method study, how to mine data ethically, and gives an overview of recent trends in MSR as well as reflects on the future. As a teaching aid, the chapter provides tips for educators, exercises for students at all levels, and a list of repositories that can be used as a starting point for an MSR study.

==> algorithms/fixed_files.tex <==
\begin{algorithm}[ht]
\caption{Procedure to identify files modified in fixing commits and their bug-inducing commits, adapted from Dalla Palma et al.~\cite{dalla2021within}.}
\label{alg:getFixedFiles}
\footnotesize
\begin{algorithmic}[1]
	\Procedure{getFixedFiles}{fixingCommits:$List[str]$}
	\State fixedFiles = []
	\State
	\For {commit \textbf{in} fixingCommits[NEWEST : OLDEST]}
	    
	    \For {file \textbf{in} commit.modifiedFiles}
	    \If{file.type != 'source code file' \textbf{or} file.changeType != 'Change'}
            \State \textbf{continue}
	    \EndIf
	    \State
	    \State bics = $SZZ(commit, file)$ \Comment Bug-Inducing Commits
        \State
	    \State currentFix = FixedFile(file.filepath, \\ 
	    \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent} 
	    \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent} 
	    fic=commit.sha, \\
	    \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent} 
	    \hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent} 
	    bic=bics[OLDEST])
	    \State
	    \If{currentFix \textbf{not in} fixedFiles}
	        \State fixedFiles.$append(currentFix)$
	    \Else
	        \State existingFix = fixedFiles.$get(currentFix)$
	        \If{currentFix.fic \textbf{is older than} existingFix.bic}
	            \State fixedFiles.$append(currentFix)$
	        \ElsIf{currentFix.bic \textbf{is older than} existingFix.bic}
	            \State existingFix.bic = currentFix.bic
	        \EndIf
	    \EndIf
	    
	    \EndFor
	\EndFor
	\State 
	\State \textbf{return} fixedFiles
	\EndProcedure
\end{algorithmic}
\end{algorithm}


==> algorithms/fixing_commits.tex <==
\begin{algorithm}[ht]
\caption{Procedure to identify defect-fixing commits,  adapted from Dalla Palma et al.~\cite{dalla2021within}.}
\label{alg:getFixingCommits}
\footnotesize
\begin{algorithmic}[1]
	\Procedure{getFixingCommits}{labels, regex}
	\State fixingCommits = []
	\State 
	\For {label \textbf{in} labels} 
	    \For {issue \textbf{in} $Repo.closedIssues(label)$}
	        \State commit = $commitClosingIssue(issue)$
	        \State fixingCommits.$append(commit.sha)$
	        %\If{Ansible files \textbf{in} commit.modifiedFiles}
	        %\EndIf
	    \EndFor 
	\EndFor
	\State
	\For {commit \textbf{in} $Repo.commits$ } 
        %\If{Ansible files \textbf{not in} commit.modifiedFiles}
        %    \State \textbf{continue}
        %\EndIf
        %\State
	    \State commit.msg.\textit{remove}(words ending with 'bug' or 'fix') 
        \If{regex \textbf{matches} commit.msg}
            \State fixingCommits.$append(commit.sha)$
        \EndIf
    \EndFor 
	
	\State 
	\State discard commits that do not modify source code files
	\State \textbf{return} fixingCommits
	\EndProcedure
\end{algorithmic}
\end{algorithm}

==> latexmkrc <==
$makeindex  = 'makeindex -s svind.ist %O -o %D %S';

$ENV{'TEXINPUTS'}='./style//:' . $ENV{'TEXINPUTS'}; 
$ENV{'BSTINPUTS'}='./style//:' . $ENV{'BSTINPUTS'}; 

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}


==> notes.tex <==
% ** Deadlines **

% As outlined in our call for chapters, we plan the following (upcoming) deadlines:

% - Submission deadline first (incomplete) draft of the chapters: December 15, 2023
% - Internal peer-review deadline and feedback to authors: January 26, 2024
% - Submission deadline revised chapter version: March 22, 2024
% - Internal peer-review deadline revised version: April 5, 2024
% - Submission deadline final chapter versions: April 19, 2024
% - Submission to publisher by editors: April 30, 2024



% https://docs.google.com/document/d/1dr16ev6ycKg_rBdihx8fwlD-f9U9444_/edit



% \section{Objective}
% In this section, we will give an overview of the chapter content and provide the motivation of how the target audience will benefit from it.

% \section{Introduction to MSR}
% In this section, we will discuss the benefits of MSR using insights and applications from MSR studies. We will also give an overview of how studies are categorized, i.e., small, medium and large-scale studies; single vs. multiple source studies (including mixed methods), their purpose, i.e., to automate vs. to learn about a topic, and the type of studies, i.e., exploratory vs. research study. 

% -What is a repo
% -Pieces of info we can mine
% -How to mine each source of info (textual, structural, historical)
% -Issues when mining – extract info from papers
% -We can do 1-3 for intro and 4/5 for data mining


% \section{Data Mining}
% In this section, we will discuss the common errors when including and excluding different types of data, the plan to ensure the quality of data when performing MSR studies, and what are the considerations for data parsing based on the type of data.






% - Bugzilla: https://www.bugzilla.org/
% - Bitbucket: https://bitbucket.org/ 
% - GitLab: https://gitlab.com/ 
% - Azure Repos: https://azure.microsoft.com/en-us/services/devops/repos/ 
% - Google Code: https://code.google.com/archive/ 
% - Jira: https://www.atlassian.com/software/jira 
% - ProjectLocker: https://www.projectlocker.com/ 
% - CloudForge: https://cloudforge.com/ 
% - Zenodo: https://zenodo.org/ 
% - Awesome GPT: https://gpt4.tools/ 
% - Docker Hub: https://hub.docker.com/
% - Kaggle: https://www.kaggle.com/ ??

% Some discussion forums include:
% - Reverse Engineering: https://reverseengineering.stackexchange.com/ 
% - Software Engineering: https://softwareengineering.stackexchange.com/ 
% - Software Quality Assurance and Test: https://sqa.stackexchange.com/ 
% - GenAI: https://genai.stackexchange.com/ —this has discussions on LLMs
% - DevOps: https://devops.stackexchange.com/ 
% - Hash Node: https://hashnode.com/ 
% - Dev: https://dev.to/p/editor_guide 
% - Code Project: https://www.codeproject.com/ 

% Some online coding platforms used by developers are:
% - Code Pen: https://codepen.io/ 
% - Replit: https://replit.com/

% 1. PyTorch Forums  ( Has a lot of discussions related to Pytorch )
% 2. Kaggle: Your Home for Data Science ( Has datasets, discussion forms, notebooks )
% 3. Hugging Face Forums - Hugging Face Community Discussion ( Hugging face discussions forum )
% 4. anon8231489123/ShareGPT_Vicuna_unfiltered · Datasets at Hugging Face ( This has 53k conversations with ChatGPT sourced by different people )



%\subsubsection{data source identification}

%Note: we will talk about the different sources but focus on GitHub for the details\\

%SO, GH issues, issue tracker systems, discussion forums, stack exchange, mailing lists, bug reports, app stores, user feedback form/forums, twitter, social media platforms (reddit, etc), \\


% 1. What Data Sources/repo? 
% categories of repo : 
% historical (version control, bugs, mailing lists, SO), 
% code (code bases, project ecosystem), 
% runtime (crash reports, field logs, execution traces)

% online judge web sites: AIZU Online Judge and AtCoder. 

% 2. Criteria for selection of the data sources/repo (perils paper)
% - for code repositories

% 3. Considerations when selecting the data sources (good, bad, avoid, best practice) - for code repositories)

% 4. shortlisting the code repo \\

% ======================================\\
% *Repositories that can be mined (some examples in ~\cite{chen2016survey})\\
% historical or runtime or code repos e.g.\\
% -source code repo\\
% -requirements/design documents\\
% -bug reports\\
% -archived communications\\
% -logs\\
% -mobile applications\\
% -developer discussions.\\

% - considerations when mining the different categories of repositories (the good, the bad, what to look out for, what to avoid, etc)\\

% - If various resources should be considered and combined to give a general view of the problem and be analyzed to provide answers. \\





% \textbf{Repository properties definition (criteria for selecting repo)}

% \textit{Munaiah, N., Kroh, S., Cabrey, C., \& Nagappan, M. (2017). Curating github for engineered software projects. Empirical Software Engineering, 22, 3219-3253.}


% \begin{itemize}
%     \item \# stars
%     \item \# contributors
%     \item \# SLOC
%     \item language 
%     \item tags (with related perils)
%     \item non-personal (e.g., only public repos for some languages), non archived ones
%     \item active repos, e.g.m considering the date of first and last commit
%     \item time of the repo creation in some applications. For example, if studying transformers issues or deep learning issues with certain frameworks, repos before the release of these models should not be considered. 
%     \item selecting the keywords (e.g., for SO) and filtering the data
%     \item number of likes, accepted answers, reputation of the user, etc.
% \end{itemize}

% considerations: \\
% -Licensing of the repos\\
% -ethics considerations, e.g., can you extract users' names and email addresses and use them in the analysis?\\
% Some repositories do not allow scraping their data, e.g., Pytorch discussion forum\\
% -consideration and context for selecting particular criteria\\
% -best practices and anti-patterns




% \subsection{General MSR pipeline}
% Then specific prediction example: How to use repo to construct recommendation systems for defect prediction
% Focus more on AI for SE tasks (go in that direction)
% Performance/sustainability aspects, etc


FHF: notes on ethics, copied from the papers.

% Much research focuses on open-source software repositories and one could assume that, as the software is published open-source, no ethics issues will arise (similar to studying published literature). However, there is a difference between the publication of source code (by intentionally applying a licence to the code itself) and the incidental public availability of
% other data (the repository) that typically lacks such a manifest act of publication. Licences
% that permit freedom to study or do not restrict the purpose of use can support an ethics
% defence for studying the code without the need for further ethics considerations. As repository data is not typically licensed like this, repository-focused studies are therefore far more
% likely to raise ethics issues than code-focused studies

% There are examples of past practices in the MSR space being revisited: email addresses
% were removed from the GHTorrent data dump in March 2016 (Baltes and Diehl 2016) and
% age information was removed from Stack Overflow’s public data as part of an audit for the GDPR (Craver 2018



% The first step in considering how ethics issues may arise in repository studies is to
% identify an appropriate ethics framework to apply, e.g. BPS (The British Psychological Society 2018, 2014), BERA2018 (British Educational Research Association 2018),
% RESPECT (Dench et al. 2004), the Menlo Report (Dittrich and Kenneally 2012), and the
% Association of Internet Researchers guidelines (Markham and Buchanan 2012; Franzke
% et al. 2020). To some extent, the choice is affected by the specific nature of the research
% problem to be addressed (e.g. some studies might be best characterised as digital social
% science, or internet-mediated social research).
% The following sections adopt the Menlo Report (Dittrich and Kenneally 2012; Bailey
% et al. 2012) as the primary ethical frame since this is a broad framework for research in the
% Information and Communication Technology space and thus can expose the set of issues to
% be considered in a relevant way. We augment the discussion with considerations from the
% two most recent AoIR ethics codes (Markham and Buchanan 2012; Franzke et al. 2020)
% that account more explicitly for the internet context of much MSR research and some of the
% issues that arise as a result.

% The Menlo Report (Dittrich and Kenneally 2012) was published in 2012 with the intention
% of providing a set of principles to help researchers identify and manage ethical issues in what
% it defines as Information and Communication Technology Research (ICTR):

% The Menlo Report sets out four principles for the consideration of ethics:
% 1. Respect for Persons (voluntary participation following informed consent; respecting
% individuals as autonomous moral agents and able to determine their own best interests;
% respect individuals impacted by, but not the targets of, research; protect those with
% limited autonomy)
% 2. Beneficence (maximise benefit; minimise harm; systematically assess risks of
% harm/benefit)
% 3. Justice (consider each individual equally; fairly distribute research benefits considering need, effort, societal contribution and merit; fairly select subjects; allocate burdens
% equitably)
% 4. Respect for Law and Public Interest (due diligence; transparency in methods and
% results; accountability).

% The Menlo Report proposes a standard method to operationalise the principles: identification of stakeholders and informed consent; balancing risks and benefits; fairness
% and equity; and compliance, transparency and accountability. 
% 4.2.1 Identification of Stakeholders
% 4.2.2 Informed Consent

% 4.2.3 Balancing Risks and Benefits: 
% MSR-type research (in common with other parts of data science) is often done with a
% mindset of “here is a dataset, let’s see what we can find”. This is potentially risky because
% the same data can be used in many ways, some safe, some risky to the participants.
% The need for ethical use of repository data (including source code and repositories themselves) is succinctly captured in the ethics policies of the Software Heritage Archive Ethical
% Charter (Software Heritage Archive 2019b) where to use the archive requires a consideration of the potential harms, the protection of personal data, and taking care of derived data and results. 

% Areas of potential harm in MSR research (and software research generally) may relate
% to observations and judgements of practices, impacting on the researched individual’s reputation, e.g. profiles of contribution rates and success, or code quality. 

% The conclusions drawn could have consequences for a developer’s ability to participate in
% future projects and may affect their ability to secure a job (Oezbek 2008). 

% 4.2.4 Fairness and Equity
% This area concerns the potential for societal contribution from the research, the fair selection
% of subjects, the availability of results, and the equitable treatment of all developers involved
% in a study. In general, these areas do not raise MSR-specific concerns. 
% Fair selection and equitable treatment may be somewhat harder to attain however. In
% research involving people, fair selection is often addressed using random sampling within
% a population. However, it is important that research is designed to be inclusive in terms of
% both questions and process, and that potential participants are not excluded for reasons other
% than the specific study exclusion criteria that apply to all.

% 4.2.5 Compliance, Transparency, and Accountability
% GDPR, CCPA, and other laws and regulations, 
% Intellectual property law
% There are many standard licences used for open source development
% The scope of compliance extends beyond laws and licensing to the terms and conditions
% of services and platforms that are used for research purposes. For example, outside of the
% MSR context but of relevance and within the scope of investigations covered by the Menlo
% Report framework, it was recently reported that Facebook has asked a group at New York
% University to cease collecting data from its site on the grounds that it has not given permission for the collection (Horwitz 2020), leading to an interesting discussion of the ethical
% balance between research needs, data subject rights, and platform rights (Naughton 2020).

5 Ethics in Mining VCS
As noted in the introduction, the code in a repository typically has a licence applied to it
by the author(s). The terms of such licences vary but those compliant with the FSF and/or
OSI licensing criteria permit study (or do not restrict use) and therefore permit research
without further reference to the authors.

Limiting research to projects with a declared licence compliant with the FSF and/or OSI
licensing criteria is perhaps the simplest approach (since these permit study and/or do not
restrict the purpose of use). Other licences would need to be considered on an individual
basis for what they permit. However, restricting MSR research to FSF/OSI compliant repositories may introduce potential bias in the same way that MSR research usually applies
selection criteria to create subsets that are analysed and where the results can only be generalised to projects that fit the selection criteria. Research that needs to generalise, e.g. to
study licensing, has a reason to not restrict the research but would need to consider the ethics
implications of doing so

5.2 Using Commit Records


=== results:
From more than 100 papers in MSR mining challenges and Data showcases from 2006 and 2014 until 2021, respectively, only a few discussed threats to validity, ethics, or anonymizing the data. 

"Moreover, they potentially demonstrate how the ethics considerations can shape projects before or while they commence, or even when projects have finished."

Guidelines on page 38


